Generalized Benders Decomposition with Continual Learning for Hybrid Model Predictive Control in Dynamic Environment

Hybrid model predictive control (MPC) with both continuous and discrete variables is widely applicable to robotic control tasks, especially those involving contact with the environment. Due to the combinatorial complexity, the solving speed of hybrid MPC can be insufficient for real-time applications. In this paper, we proposed a hybrid MPC solver based on Generalized Benders Decomposition (GBD) with continual learning. The algorithm accumulates cutting planes from the invariant dual space of the subproblems. After a short cold-start phase, the accumulated cuts provide warm-starts for the new problem instances to increase the solving speed. Despite the randomly changing environment that the control is unprepared for, the solving speed maintains. We verified our solver on controlling a cart-pole system with randomly moving soft contact walls and show that the solving speed is 2-3 times faster than the off-the-shelf solver Gurobi.

==> sect_theoretical_analysis.tex <==
In this section, we present some theoretical guarantees for convergence and solving speed with Benders decomposition. 

\subsection{Global convergence}

We first give a guarantee that this algorithm converges to the global optimal $\boldsymbol{z}$.

\begin{lemma}
Let $X^*(\boldsymbol{x}_{ini})$ be the set of global optimal solution pairs $(\boldsymbol{x}^*, \boldsymbol{z}^*)$ under given $\boldsymbol{x}_{ini}$. Let the projection of $X^*$ onto the $\boldsymbol{z}^*$ space be $Z^*$. The algorithm terminates immediately after it picks out $\boldsymbol{z}^* \in Z^*$.
\end{lemma}
\begin{proof}
Since it is global optimal, the upper bound cannot be lower. The Lagrange multiplier should be zero at this point. Note the nonconvexity.
\end{proof}

The convergence to global optimal solution is a natural result from that $Z^*$ is a countable many set, and any iteration in the process does not remove global optimal solutions otherwise the algorithm terminates immediately. Despite its simplicity, we invoke the theorem of countable many sets to formally states the assumptions.

\begin{theorem}
(Global convergence).
\end{theorem}
\begin{proof}
\end{proof}

\subsection{Guarantee of feasibility via extreme ray enumeration}
We then quantify the running speed of the proposed algorithm. We begin with some preliminary results. 

\begin{lemma}
The dual feasible set of ~\eqref{Eqn:Infeasible_dual} is a pointed cone.
\end{lemma}
\begin{proof}
% Show that the subspace $\nu$ cannot contain a full line. If there is a $\delta \nu$ that breaks the equality, $\lambda$ has to somehow handle it (otherwise a line of $\delta \nu$ cannot exist), but that makes $\lambda$ breaking the non-negativity condition. Then 
The dual feasible set of ~\eqref{Eqn:Infeasible_dual} can be written as:

\begin{equation}
    \begin{bmatrix}
         \boldsymbol{A}^T & \boldsymbol{C}^T \\
        -\boldsymbol{A}^T & -\boldsymbol{C}^T \\
         \boldsymbol{0}   & \boldsymbol{I}
    \end{bmatrix} 
    \begin{bmatrix}
    \boldsymbol\nu \\
    \boldsymbol\lambda
    \end{bmatrix} \geq \boldsymbol{0}
\end{equation}

The square submatrix:
\begin{equation}
\begin{aligned}
\begin{bmatrix}
\boldsymbol{I}_{n_{x}} & -\boldsymbol{E}            &                         &    & \boldsymbol{L} \\
                   &                 \ddots & \ddots                  &    & & \ddots \\
                   &                        & \ \  \boldsymbol{I}_{n_{x}} & -\boldsymbol{E} & & & \boldsymbol{L} \\
                   &                        &                         & \ \  \boldsymbol{I}_{n_{x}} \\
                   &                        &                         &    & \ \  \boldsymbol{I}_{n_{c}} \\
                   &                        &                         &    & & \ddots \\
                   &                        &                         &    & & & \boldsymbol{I}_{n_{c}} \\
\end{bmatrix} \\
\in \mathbb{R}^{((N+1)n_x + Nn_c) \times ((N+1)n_x + Nn_c)}
\end{aligned}
\end{equation}

Has $(N+1)n_x + Nn_c$ linearly independent rows. Then apply theorem 4.12(c) in \cite{bertsimas1997introduction}.
\end{proof}

Given that the dual cone is pointed, we can guarantee feasibility by enumerating all extreme rays. When solving problem ~\eqref{Eqn:infeasible_MLD}, it is important to use the dual simplex method. As indicated by \cite{bertsimas1997introduction}, $\tilde{\boldsymbol\nu}_{p}$, $\tilde{\boldsymbol\lambda}_{p}$ returned by dual simplex are extreme rays if the problem is infeasible. We further present:

\begin{lemma}
$\tilde{\boldsymbol\nu}_p^m$, $\tilde{\boldsymbol\lambda}_p^m$ are extreme rays for any $m$.
\end{lemma}
\begin{proof}
As $\tilde{\boldsymbol\nu}_p^m$, $\tilde{\boldsymbol\lambda}_p^m$ are dual feasible, they are rays since any positive scaling of them are still dual feasible. By shifting, all equality constraints remains active. Comparing to the original inequality constraints, $\tilde{\boldsymbol\lambda}_{p,0} \geq \boldsymbol{0}$ is removed at $t=0$ and $\tilde{\boldsymbol\lambda}_{p,N-1} = \boldsymbol{0} \geq \boldsymbol{0}$ is added at $t=N-1$. Since the added constraints are all active, the number of linearly independent constraints at $\tilde{\boldsymbol\nu}_p^m$, $\tilde{\boldsymbol\lambda}_p^m$ do not decrease \xuan{Should show the matrix form otherwise the new active constraints could be linearly dependent!}. The conclusion follows by definition 4.2 of \cite{bertsimas1997introduction}.  
\end{proof}

Recall the equivalence of extreme rays and the complete set of extreme rays given that they have finite many from \cite{bertsimas1997introduction}:
\begin{definition}
Two extreme rays are equivalent if one is a positive multiple of the other.    
\end{definition}

\begin{definition}
A finite collection of extreme rays is a complete set of extreme rays if it contains exactly one representative from each equivalent class.   
\end{definition}

As the cone is pointed and we minimize $\boldsymbol\nu^{T}\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z}_p) + \boldsymbol\lambda^{T}\boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z}_p)$ over the cone, if the cost is $-\infty$ then there exist some extreme ray $\tilde{\boldsymbol\nu}$, $\tilde{\boldsymbol\lambda}$ of the cone such that $\tilde{\boldsymbol\nu}^{T}\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z}_p) + \tilde{\boldsymbol\lambda}^{T}\boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z}_p)<0$ by Theorem 4.13 \cite{bertsimas1997introduction}. If we have added a feasibility cut of the form $\tilde{\boldsymbol\nu}^{T}\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z}) + \tilde{\boldsymbol\lambda}^{T}\boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z}) \geq 0$ for all extreme rays, feasibility is guaranteed by the master problem. Note that all extreme rays are required to prove infeasibility for any infeasible solution.

\begin{lemma}
(All extreme rays are useful) \xuan{This theorem is a little too in detail, put in appendix if needed.} Let $\boldsymbol{r}_0, ..., \boldsymbol{r}_n$ be the complete set of extreme rays for the dual feasible cone of ~\eqref{Eqn:Infeasible_dual}. The cost of is optimization problem is $-\infty$: 
\begin{equation}
\begin{aligned}
    &\underset{\boldsymbol{x}_{ini}, \boldsymbol{z}}{\text{minimize}} \ \ \matt{\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z})^T & \boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z})^T} \cdot \boldsymbol{r}_j\\
    \text{s.t.} \ \ & \matt{\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z})^T & \boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z})^T} \cdot \boldsymbol{r}_i \geq 0 \ \ i=0,...,n, i \neq j\\
\end{aligned}
\end{equation}
Or if any extreme ray is $\boldsymbol{r}_j$ is not added to the feasibility cuts, we can find some $\boldsymbol{x}_{ini}, \boldsymbol{z}$ such that the subproblem is infeasible.
\end{lemma}
\begin{proof}
A little lengthy. Should put in the appendix. Is there a more concise way to show this? Also, \xuan{Strong duality still remains to be justified!}
\end{proof}

As they are all extreme rays, as long as they are not equivalent to the existing ones, they contribute to eliminating infeasible solutions, despite the value of $\boldsymbol{z}$ and $\boldsymbol{x}_{ini}$. \xuan{Explain that the equivalence only need to be checked at the same level of cone}. Therefore, we keep all non-equivalent extreme rays in the algorithm. As extreme rays are finite many, in theory, we can enumerate all of them and feasibility is guaranteed. This gives a bound of control delay even if the dynamics is changed.

\begin{lemma}
(Bounded delay from zero start) The algorithm returns a feasible solution within xx iterations.
\end{lemma}
\begin{proof}
Use the max number of extreme rays. This bound may be bad. Maybe you should do it throughout several iterations.
\xuan{Does the nonuniqueness of the optimal $\boldsymbol{z}$ cause some trouble for this analysis?}
\end{proof}

The theoretical bound is bad. However, this algorithm works fairly well from zero start for the problems that we have tested.

\subsection{Reuse of feasibility cuts for different initial conditions}
This theoretical bound can be bad. However, we almost never reach this bound in practice. We note the role of master problem in terms of enumerating infeasible proofs. Its role is 2-fold: it removes certain $\boldsymbol{z}$'s are infeasible, but also simultaneously finds the most optimal $\boldsymbol{z}$'s given its current limited understanding of the subproblem from the optimality cuts. This justifies the efficiency of Benders decomposition for enumerating extreme rays: despite the vast number of extreme rays, it never needs to enumarate all of them, only the ones that has good optimal costs from optimality cuts. Therefore, if the new $\boldsymbol{x}_{ini}^{\prime}$ is not very different from one of the previous $\boldsymbol{x}_{ini}$, the optimality will also be not very different and all the enumeration computations can be reused.

We first investigate the conditions under which the feasibility cuts collected with initial condition $\boldsymbol{x}_{ini}$ can all be reused for a new initial condition $\boldsymbol{x}_{ini}^{\prime}$. We note that the new initial condition does not need to happen at the next time step.

Assume that when the algorithm investigate initial condition $\boldsymbol{x}_{ini}$, it investigated infeasible $\boldsymbol{z}_s, \ s=1,...,S$ before reaching the global optimal solution $\boldsymbol{z}^*$, during this process the following feasibility cuts are created:

\begin{equation}
\boldsymbol{b}(\boldsymbol{x}_{ini}, \boldsymbol{z})^{T} \tilde{\boldsymbol\nu}_{s} + \boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z})^{T} \tilde{\boldsymbol\lambda}_{s} \geq 0, \ s=1,...,S
\end{equation}

\xuan{(the cuts may not be enumerated by $\boldsymbol{x}_{ini}$ but even previous iterations?)}

Under new initial condition $\boldsymbol{x}_{ini}^{\prime}$, 2 conditions need to be true such that we do not need to enumerate new cuts. First, the optimality of $\boldsymbol{z}$'s should not change too much, so the $\boldsymbol{z}$'s needed to be investigated by the master problem are still $\boldsymbol{z}_s, \ s=1,...,S$ and we do not need to explore any new $\boldsymbol{z}$. Second, the existing cutting planes are still valid for those $\boldsymbol{z}$ under the new $\boldsymbol{x}_{ini}^{\prime}$. Those 2 conditions confine relations between $\boldsymbol{x}_{ini}$ and $\boldsymbol{x}_{ini}^{\prime}$.

For the optimality of $\boldsymbol{z}$'s not changing too much, we want no $\boldsymbol{z}$'s other than $\boldsymbol{z}_s$ to have better optimal cost than the current $\boldsymbol{z}^{*\prime}$ under the optimal cuts. Let $\Delta \boldsymbol{x}_{ini} \triangleq \boldsymbol{x}_{ini}^{\prime} - \boldsymbol{x}_{ini}$. We make an assumption of Lipschitz continuity on $\boldsymbol{x}_{ini}$:

\begin{assumption}
(Lipschitz condition) The optimal cost function $v(\boldsymbol{x}_{ini}, \boldsymbol{z})$ satisfies:
\begin{equation}
    |v(\boldsymbol{x}_{ini}^{\prime}, \boldsymbol{z}) - v(\boldsymbol{x}_{ini}, \boldsymbol{z})| \leq L||\Delta \boldsymbol{x}_{ini}||
\end{equation}
\end{assumption}

Due to the Lipschitz condition, the optimal cost changes no more than $L||\Delta \boldsymbol{x}_{ini}||$ if feasibility does not change. This also gives a bound of the dual gap:

\begin{corollary}
    Let the optimal gap be defined by $g(\boldsymbol{x}_{ini}, \boldsymbol{z}) = v(\boldsymbol{x}_{ini}, \boldsymbol{z})-z_0$, where $z_0$ minimizes the optimality cuts:
    \begin{equation}
    \begin{aligned}
        &\underset{\boldsymbol{z}}{\text{minimize}} \ \ z_0 \\
        \text{s.t.}
        & \ \text{for} \ \forall q \ \text{the subproblem is feasible under $\boldsymbol{x}_{ini}$} \\
        & z_0 \geq f_{obj,q}^* + \boldsymbol\nu_{q}^{*T} (\boldsymbol{b}(\boldsymbol{x}_{ini}, \boldsymbol{z}_q) - \boldsymbol{b}(\boldsymbol{x}_{ini}, \boldsymbol{z})) + \\
        & \ \ \ \ \ \ \ \boldsymbol\lambda_{q}^{*T} (\boldsymbol{d}(\boldsymbol{z}_q)-\boldsymbol{d}(\boldsymbol{\theta},\boldsymbol{z})) \\ 
    \end{aligned} 
    \end{equation}
For any feasible $\boldsymbol{z}_{q}$ under $\boldsymbol{x}_{ini}$, we have:
\begin{equation}
    0 \leq g(\boldsymbol{x}_{ini}^{\prime}, \boldsymbol{z}_q) \leq L||\Delta \boldsymbol{x}_{ini}|| + \boldsymbol\nu_{q,0}^{*T}\Delta \boldsymbol{x}_{ini}
\label{Eqn:dual_gap_pf}
\end{equation}
\end{corollary}

\xuan{LHS has to be 0?}

\begin{proof}
Due to strong duality, $z_0 = f_{obj,q}^* = v(\boldsymbol{x}_{ini}, \boldsymbol{z})$. At $\boldsymbol{x}_{ini}^{\prime}$, $z_0 \geq v(\boldsymbol{x}_{ini}, \boldsymbol{z}) - \boldsymbol\nu_{q,0}^{*T}\Delta \boldsymbol{x}_{ini}$ due to constraint satisfaction. Given that $v(\boldsymbol{x}_{ini}^{\prime}, \boldsymbol{z}_q) \leq v(\boldsymbol{x}_{ini}, \boldsymbol{z}_q) + L||\Delta \boldsymbol{x}_{ini}||$ via Lipschitz condition, ~\eqref{Eqn:dual_gap_pf} follows.   
\end{proof}

Two conditions are required:

\begin{enumerate}
    \item For any $\boldsymbol{z}$ other than $\boldsymbol{z}_s$, the optimal cost is worse than $v(\boldsymbol{x}_{ini}, \boldsymbol{z}_s)$ by at least $\Delta v$ (for now, just state that this $\Delta v$ exists without referring to its actual value).
    \item The optimal $\boldsymbol{z}^*$ remains to be feasible under $\boldsymbol{x}_{ini}^{\prime}$.
\end{enumerate}

Under those conditions, the following equation ensures that no other $\boldsymbol{z}$ needs to be explored:

\begin{equation}
    3L||\Delta \boldsymbol{x}_{ini}|| + \boldsymbol\nu_{q,0}^{*T}\Delta \boldsymbol{x}_{ini} \leq \Delta v
\end{equation}

For the existing cutting planes to be valid under the new $\boldsymbol{x}_{ini}^{\prime}$, we need the following to be valid:

\begin{equation}
\boldsymbol{b}(\boldsymbol{x}_{ini}^{\prime}, \boldsymbol{z}_s)^{T} \tilde{\boldsymbol\nu}_{s} + \boldsymbol{d}(\boldsymbol{z}_s)^{T} \tilde{\boldsymbol\lambda}_{s} < 0, \ s=1,...,S
\label{Eqn:reuse_feasibility_cuts}
\end{equation}

Let $\epsilon_s>0$ be the gap for the original cuts with $\boldsymbol{z}_s$, such that $\boldsymbol{b}(\boldsymbol{x}_{ini}, \boldsymbol{z}_s)^{T} \tilde{\boldsymbol\nu}_{s} + \boldsymbol{d}(\boldsymbol{z}_s)^{T} \tilde{\boldsymbol\lambda}_{s} + \epsilon_s = 0$.  Therefore, we have the condition for ~\eqref{Eqn:reuse_feasibility_cuts} to be valid:

\begin{equation}
    \Delta \boldsymbol{x}_{ini}^T \tilde{\boldsymbol\nu}_{s,0} \leq \epsilon_s
\end{equation}

This inequality is a sufficient condition to guarantee that $\boldsymbol{z}_s$ is still infeasible for $\boldsymbol{x}_{ini}^{\prime}$, but not necessary, as $\boldsymbol{z}_s$ can violate multiple extreme rays.

\begin{equation}
    -\eta^* \leq \Delta \boldsymbol{x}_{ini}^T \tilde{\boldsymbol\nu}_{\eta,0}
\end{equation}

$\eta^* \geq 0$ is the extreme ray in the dual feasible cone that minimizes $\tilde{\boldsymbol\nu}^{T}\boldsymbol{b}(\boldsymbol{x}_{ini}, \ \boldsymbol{z}^*) + \tilde{\boldsymbol\lambda}^{T}\boldsymbol{d}(\boldsymbol{z}^*)$.

This condition gives a linear region of $\boldsymbol{x}_{ini}^{\prime}$, speaking that $\boldsymbol{z}^*$ remains feasible but more optimal $\boldsymbol{z}_q$'s remain infeasible. 

With the warm-start, we can investigate the optimality in the next iteration. As the algorithm proceeds, the dual gap will keep on reducing. If the dual gap can be bounded and one feasible solution can be founded within one iteration, then we can find a mode sequence that decreases the cost hence stabilizes the system within one trial. We call this one shot stable.

\begin{lemma}
    (One shot stable) If the dual gap is bounded within $\epsilon$, then the next iteration, BD finds a mode sequence that decreases the cost hence stabilizes the system.
\end{lemma}
\begin{proof}
    \xuan{Be careful that definition of stability is for both x and z, check Bemporad paper!}
    Assume there is no noise. In this iteration, an optimal mode sequence is $\boldsymbol{z}$. Then in the next iteration, the contact sequence $\boldsymbol{z}_s$ is a feasible one that will decrease the cost by $v(\boldsymbol{x}_{1}, \boldsymbol{z})-v(\boldsymbol{x}_{ini}, \boldsymbol{z}_s)$. As the master problem finds optimal solution based on optimality cuts, and none of the feasible solutions will be cut out, if $\epsilon \leq (v(\boldsymbol{x}_{1}, \boldsymbol{z})-v(\boldsymbol{x}_{ini}, \boldsymbol{z}_s))$, then the mode sequence cannot have a cost worse than this iteration (when next iteration the dual gap is maximal and this iteration the dual gap is 0). Stability is a result from that the cost decrease (use cost as a Lyapunov function).
\end{proof}

\subsection{Asymptotic analysis for MPC}
Specialize the previous section for MPC analysis.

\xuan{How does the model error affects the algorithm? As such, how does this method perform under unseen scenarios so it beats KNN based methods? Study under what noise condition are those old cuts still valid for the new $\boldsymbol{x}_{ini}$? Is this stronger than the asymptotic conditions for Tobia's paper?} 

